Learning Adversary Behavior in Security Games: A PAC Model Perspective

Recent applications of Stackelberg Security Games (SSG), from wildlife crime to urban crime, have employed machine learning tools to learn and predict adversary behavior using available data about defender-adversary interactions. Given these recent developments, this paper commits to an approach of directly learning the response function of the adversary. Using the PAC model, this paper lays a firm theoretical foundation for learning in SSGs (e.g., theoretically answer questions about the numbers of samples required to learn adversary behavior) and provides utility guarantees when the learned adversary model is used to plan the defender's strategy. The paper also aims to answer practical questions such as how much more data is needed to improve an adversary model's accuracy. Additionally, we explain a recently observed phenomenon that prediction accuracy of learned adversary behavior is not enough to discover the utility maximizing defender strategy. We provide four main contributions: (1) a PAC model of learning adversary response functions in SSGs; (2) PAC-model analysis of the learning of key, existing bounded rationality models in SSGs; (3) an entirely new approach to adversary modeling based on a non-parametric class of response functions with PAC-model analysis and (4) identification of conditions under which computing the best defender strategy against the learned adversary behavior is indeed the optimal strategy. Finally, we conduct experiments with real-world data from a national park in Uganda, showing the benefit of our new adversary modeling approach and verification of our PAC model predictions.

==> Notation_old.tex <==
This section introduces the background and a summary of notations (Table \ref{Table1}) for this paper. Given two $n$-dimensional points $M$ ($m_1, \ldots, m_n$) and $M'$ ($m'_1, \ldots, m'_n$), we define the $l_p$ distance metric $d_{l_p}$ between the two points as: $d_{l_p}(M,M') =||M - M'||_p = (\sum_i |m_i - m'_i|^p)^{1/p}$. In particular, $d_{l_\infty}(M,M') = ||M - M'||_\infty = \max_i |m_i - m'_i|$. Also $d_{\bar{l_p}} =  d_{l_p}/n$. The notation $M \cdot M'$ denotes the dot product between two vectors.

\subsection{Stackelberg Security Games}
\label{sec:SSG}

We focus on Stackelberg Security Games (SSG) in this paper, however, our results generalize to Stackelberg games as well (see Appendix). An SSG %security game 
is a two player Stackelberg game between a defender and an adversary --- the defender plays the role of a leader who protects a set of targets from the adversary who acts as the follower \cite{Conitzer2006,Paruchuri2008}. %\cite{Conitzer2006,Paruchuri2008,Korzhyk10}. 
The defender wishes to protect $T$ targets with a limited number of security resources $K$ ($K <\!< T$). %resources. 
For ease of presentation, we restrict ourselves to the scenario with no scheduling constraints~\cite{}. The defender's pure strategy is to allocate each resource to a target. %, while the adversary's pure strategy is to attack a single target. 
%Therefore, there are $T \choose K$ possible pure strategies for the defender. %and $T$ possible pure strategies of the adversary. 
A defender's mixed-strategy $\tilde x$ ($0\leq \tilde x_{j}\leq 1; \forall \tilde x_{j}, j\in P; \sum_{j=1}^{P}\tilde x_{j}=1)$ is then defined as a probability distribution over the set of all possible pure strategies $P$. An equivalent description \cite{Korzhyk10,yang:ijcai2011} of these mixed strategies is a probability distribution over the set of targets: $x$ ($0\leq x_{i}\leq 1; \forall x_{i}, i\in T; \sum_{i=1}^{T}x_{i}=M)$. In the rest of this article, we will refer to this latter description as the mixed strategy of the defender.
%The defender's pure strategies can be represented as a $0,1$ vector of size $T$, where $1$ in position $i$ $(i\in T)$ indicates that target $i$ is protected. The defender's mixed strategy can be represented by the vector $\tilde x$ of size $T \choose K$, where each component $\tilde x_j$ gives the probability of deploying pure strategy $j; j=1...$$T\choose K$. Let $D$ be a matrix of size $T$ $\times$ $T \choose K $, i.e., each row of $D$ denotes a target and each column denotes a pure strategy for the defender. Then, the defender's mixed strategy can be succinctly expressed as numbers $x_1, \ldots, x_T$ with $0 \leq x_i \leq 1$ such that $x = D\tilde x$. Intuitively, $x_i$ denotes the probability of defending target $i$. Let this space of marginal mixed strategies of the defender be $X$. In earlier work~\cite{}, it has been shown that $X$ can be described by $0 \leq x_i \leq 1$ and $\sum_i x_i \leq K$. 

A pure strategy of the adversary is defined as attacking a single target. The adversary's mixed strategy is then a categorical distribution over the set of targets. Thus, it can be expressed as parameters $q_i$ $(i\in T)$ of the categorical distribution such that $0 \leq q_i \leq 1$ and $\sum_i q_i = 1$.  The adversary's response to the defender's %marginal 
mixed strategy is given by a function $q: X \rightarrow Q$, where $Q$ is the space of mixed strategy of the adversary. As is common in games, a matrix $U$ specifies the payoffs of the defender, and her expected utility is $x^T U q(x)$ when she plays a %marginal 
mixed strategy $x \in X$. 
%The defender aims to learn $h$, in order to obtain maximum utility.
%In this paper, our aim is characterize the learning complexity for different classes $\mathcal{H}$ of the function $h$, and provide bounds on the utility for the defender in each case.

\subsection{Bounded Rationality Models}
\label{sec:boundedRationality}

Although a perfectly rational adversary would choose to attack the target with highest expected utility, recent work has focused on modeling boundedly rational adversaries in SSGs -- the most relevant one is discussed below.

\noindent \textbf{Subjective Utility Quantal Response (SUQR)}:
%\label{sec:suqr}
SUQR \cite{Nguyen13analyzingthe} builds upon prior work on quantal response \cite{McFadden1976} according to which rather than strictly maximizing utility, an adversary stochastically chooses to attack targets, i.e., the adversary attacks a target with higher expected utility with a higher probability. Formally, according to the QR model, given $n$ actions, with each action $i$ yielding utility $U_i$, the player plays action $i$ with probability $q_i \propto e^{\lambda U_i}$, where $\lambda$ is a parameter. SUQR extends the QR model by using \emph{subjective utility} instead of $\lambda U_i$ in the expression for $q_i$ above. The subjective utility is defined as $w \cdot v$, where $v$ denote values of a set of features and $w$ denotes the weight parameters for these features. This is based on the Lens model in psychology which is a framework for modeling prediction based on observable cues \cite{Brunswik1952,Hammond1955}. The features are specific to the domain, for example, in case of standard security game applications, the set of features may include the coverage probability $x_i$ and the reward and penalty of target $i$. Since, other than the coverage, remaining features are fixed in real world data, we analyze the following parametric form of SUQR with parameters $w_1$ and $c_i$'s: $q_i \propto e^{w_1 x_i + c_i}$. Since SUQR and its variants have been shown to perform the best among competing bounded rationality models, we will use SUQR and its above mentioned parametric form as the basis for our analysis. 
%Thus, according to this model, the probability that the adversary will attack target $i$ is given by:
%\begin{equation}
%%\vspace{-1pt}
%%q_{i}(\omega|x)=\frac{e^{SU_{i}^{a}(x)}}{\underset{j\in\mathbb{T}}{\sum}e^{SU_{j}^{a}(x)}}
%%\label{attackProb_suqr}
%q_{i}(\omega|x)=\frac{e^{SU_{i}^{a}(x)}}{\underset{j\in T}{\sum}e^{SU_{j}^{a}(x)}}
%\label{attackProb_suqr}
%%\vspace{-1pt}
%\end{equation}
%where $SU_{i}^{a}(x)$ is the Subjective Utility of an adversary for attacking target $i$ when defender employs strategy $x$ and is given by:
%\begin{equation}
%%\vspace{-1pt}
%SU_{i}^{a}(x)=\omega_{1}x_{i}+\omega_{2}R_{i}^{a}+\omega_{3}P_{i}^{a}
%\label{SU}
%%\vspace{-1pt}
%\end{equation}
%%The reward and penalty for the attacker for attacking target $t$ are $R_{t}^{a}$ and $P_{t}^{a}$ respectively. $x_{t}$ is the coverage probability for target $t$. %Also note that $\sum_{t\in\mathbb{T}}q_{t}\left(\omega\,\vert\, x\right)=1$. 
%The vector $\omega=\left(\omega_{1},\omega_{2},\omega_{3}\right)$ encodes information about the adversary's behavior and each component of $\omega$ indicates the relative importance the adversary gives to each attribute in the decision making process. The weights are computed by performing Maximum Likelihood Estimation (MLE) on available attack data.

%\subsection{PAC learning}
\section{Learning Framework}
\label{sec:pacLearning}

\begin{table}
\begin{tabular}{l| l}
Notation & Meaning\\
\hline
$d_{l_p}(M, M')$ & $l_p$ distance between points $M,M'$ \\
$d_{\bar{l_p}}(M, M')$ & Average $l_p$ distance: $=d_{l_p}(M, M')/n$ \\
$T$ & Number of targets \\
$K$ & Number of defender resources \\
$X$ & Instance space (defender mixed strategies) \\
$Y$ & Outcome space (attacked target) \\
$A$ & Decision space \\%(attack prediction) \\
$h \in \mathcal{H}$ & $h:X \rightarrow A$ is the hypothesis function \\
$\mathcal{N}(\epsilon, \mathcal{H}, d)$ & $\epsilon$-cover of set $\mathcal{H}$ using distance $d$\\
$\mathcal{C}(\epsilon, \mathcal{H}, d)$ & capacity of $\mathcal{H}$ using distance $d$\\
$r_h(p), \hat{r}_h(\vec{z})$ & risk, empirical risk of hypothesis $h$\\
$d_{L^1(P, d)} (f, g)$ & $L_1$ distance between functions $f,g$\\
$q^p(x)$ & parameters of true categorical distr.\\
$q^h(x)$ & parameters of categorical distr. due to $h$\\
\end{tabular}
\caption{Notations}
\label{Table1}
\end{table}

We use the learning framework of Haussler~\shortcite{Haussler1992}. We define our \emph{instance space} $X$ to be the same as the space of defender mixed strategies $x\in X$. \emph{Outcome space} $Y$ is defined as the space of all possible categorical choices over a set of $T$  targets (i.e., choice of target to attack) for the adversary: %$\{y_1, \ldots, y_T\}$ 
$(y_1, \ldots, y_T)$ ($y_i \in \{0,1\}, \sum_i y_i = 1$). To give an example, given two targets $T_1$ and $T_2$, $Y=\{(0,1),(1,0)\}$, where $(0,1)$ denotes that $T_1$ was not attacked while $T_2$ was attacked, and so on. The training data are samples drawn from $Z = X\times Y$ using an unknown distribution, say given by density $p(x,y)$, i.e., each training data point denotes the adversary's response (attack on a target) to a particular defender mixed strategy. Haussler~\shortcite{Haussler1992} also defines a \emph{decision space} $A$, %(predictions), 
a \emph{space of hypothesis} (functions) $\mathcal{H}$ with elements $h:X \rightarrow A$ and a \emph{loss function} $l:Y \times A \rightarrow \mathbb{R}$. 
Given our choice of the parametric SUQR model described in the Background section, $A$ would be the space of all vectors of the following form: $<w_1 x_1 + c_1, w_1 x_2 + c_2, ... , w_T x_T + c_T>$ ; $\forall x\in X$. $\mathcal{H}$ would be the space of all mappings from defender mixed strategies $x\in X$ to $a\in A$. The loss function captures the loss of predicting attack probabilities based on the learned $a$'s when the actual outcomes are given by $y\in Y$. %Details of the loss function used for our analysis is presented in the next section. 
%The loss function captures the loss when the prediction is $a\in A$ and the actual outcome is $y\in Y$. 
The learning algorithm aims to learn a hypothesis in $\mathcal{H}$ that minimizes the expected loss (defined in next paragraph). These sets and functions (for example, the loss function) are specific to problems and we will define them subsequently for different cases. 

The \emph{true risk} of a particular hypothesis (predictor) $h$, given density function $p(x,y)$ over $Z$, %$X \times Y$,
is defined as the expected loss of predicting outcome $y$ as $h(x)$:
$$r_h (p) = \int p(x,y) l(y,h(x)) \, dx \, dy $$
The \emph{empirical risk} $\hat{r}_h(\vec{z})$, where $\vec{z}$ is a sequence of $s$ training samples from $Z$, is defined as: $\hat{r}_h(\vec{z}) = 1/s \sum_{i=1}^s l(y_i, h(x_i))$. Let $h^*$ be the hypothesis that minimizes the true risk, i.e., $r_{h^*}(p) = \inf \{r_h(p) ~|~ h \in \mathcal{H}\}$ and let $\hat{h}^*$ be the hypothesis that minimizes the empirical risk, i.e., $\hat{r}_{\hat{h}^*}(\vec{z}) = \inf \{\hat{r}_h(\vec{z}) ~|~ h \in \mathcal{H}\}$. The following is a well-known result for any \emph{empirical risk minimizing} algorithm $\mathcal{A}$ yielding hypothesis $\mathcal{A}(\vec{z})$:
$$
\begin{array}{c}
\mbox{If }Pr(\forall h \in \mathcal{H}. |\hat{r}_h(\vec{z}) - r_h(p)| < \alpha/3 ) > 1 - \delta/2\\
\mbox{and } Pr(|\hat{r}_{\mathcal{A}(\vec{z})}(\vec{z}) - \hat{r}_{\hat{h}^*}(\vec{z})| < \alpha/3 ) > 1 - \delta/2\\
\mbox{then } Pr( |r_{\mathcal{A}(\vec{z})}(p) - r_{h^*}(p)| < \alpha ) > 1 - \delta
\end{array}
$$
The space $\mathcal{H}$ is called $(\alpha, \delta)$-learnable if there exists an algorithm $\mathcal{A}$ such that the two pre-conditions are satisfied. The second pre-condition is assumed to hold, due to the performance guarantee of $\mathcal{A}$. Thus, we will focus on finding the bounds for the first pre-condition. 

In order to obtain bounds on the first pre-condition, we define \emph{covering number} and \emph{capacity} of function spaces. Let $d$ be a pseudo metric on any set $S$. For any $\epsilon > 0$, an $\epsilon$-cover for set $T \subseteq S$
is a finite set $N\subseteq S$  such that for all $x \in T$
there is a $y \in N$ with $d(x, y) \leq \epsilon$.
The \emph{covering number} $\mathcal{N}(\epsilon, T, d)$ denotes the size of the
smallest $\epsilon$-cover for set $T$ (for the pseudo metric d). We will focus on covering numbers for $\mathcal{H}$, the first step of which is to define a pseudo metric on $\mathcal{H}$. The following is a pseudo metric on $A$: $$\begin{array}{c}\rho(a, b) = \max_i |l(y_i, a) - l(y_i, b)|. \end{array}$$ Any pseudo metric $d$ on $A$ induces a pseudo metric $d_{L^1(P, d)}$ on $\mathcal{H}$ for any probability measure $P$ on $X$ and is given by
$$
\begin{array}{c}
d_{L^1(P, d)} (f, g) = \int_X d(f(x), g(x)) \; dP(x)
\end{array}
$$
For notational ease, when $d$ is not written in the subscript, e.g., $d_{L^1(P)} (f, g)$, then $d$ is assumed to be $d_{l_1}$.
%\begin{definition} \label{capacity}
The \emph{capacity} $\mathcal{C}(\epsilon, \mathcal{H}, d)$ is defined as:
$$
\mathcal{C}(\epsilon, \mathcal{H}, d) = \sup_P \; \{\mathcal{N}(\epsilon, \mathcal{H}, d_{L^1(P, d)})\}
$$

Haussler proposes pseudo-dimension $dim_P (\mathcal{H})$ as the generalization of the concept of VC dimension. In particular, they prove that if the space of functions $\mathcal{H}$ forms a vector space of dimension $l$, then $dim_P (\mathcal{H})= l$ (Theorem 4). Also, combining Theorem 6, 12 in \cite{Haussler1992} and the definition of capacity $\mathcal{C}$ we can readily infer that for any hypothesis space $\mathcal{H}$ with real valued functions and $dim_P (\mathcal{H})= l$ 
\begin{equation} \label{1dbound}
\mathcal{C}(\epsilon, \mathcal{H}, d_{l_1}) < 2 \Big( \frac{2eM}{\epsilon} \log \frac{2eM}{\epsilon} \Big)^{l}
\end{equation}

In general, if the pseudo-dimension is finite, the above equation provides a sharper bound that using the related concept of fat-shattering dimension (see Bartlett et al.~\shortcite{}).
Below is a minor modification of Theorem 9 \cite{Haussler1992}:
\begin{theorem} \label{PACbound}
Assume that the hypothesis space $\mathcal{H}$ is permissible\footnote{As noted in Haussler: ``This is a measurability condition defined in Pollard (1984) which need not concern us in
practice.''}. Let $P$ be any probability distribution on
$Z=X\times Y$. Assume that $m\geq 1$ and $0< \epsilon<1$. Let $\vec{z}$ be generated by $m$
independent draws from $Z$ according to $P$. Then
$$Pr(\forall h \in \mathcal{H}. |\hat{r}_h(\vec{z}) - r_h(p)| < \alpha) \geq 1- 4\mathcal{C}\Big(\frac{\alpha}{16}, \mathcal{H}, \rho \Big)e^{-\frac{\alpha^2m}{64M^2}}$$
\end{theorem}
\begin{proof}
Choose $\alpha = \alpha'/4M$ and $\nu = 2M$ in Theorem 9 of \cite{Haussler1992}. Using property (3) (Section 2.2, \cite{Haussler1992}) of $d_v$ we obtain $|r - s| \leq \epsilon$ whenever $d_v(r, s) \leq \alpha'$. Using this directly in Theorem 9 of Haussler~\shortcite{Haussler1992} we obtain the desired result above.
\end{proof}




